Fantasizing with Dual GPs in Bayesian Optimization and Active Learning

Gaussian processes (GPs) are the main surrogate functions used for sequential modelling such as Bayesian Optimization and Active Learning. Their drawbacks are poor scaling with data and the need to run an optimization loop when using a non-Gaussian likelihood. In this paper, we focus on `fantasizing' batch acquisition functions that need the ability to condition on new fantasized data computationally efficiently. By using a sparse Dual GP parameterization, we gain linear scaling with batch size as well as one-step updates for non-Gaussian likelihoods, thus extending sparse models to greedy batch fantasizing acquisition functions.

==> fig/lunar/lunar_lander_probability.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}

\begin{axis}[
height=\figureheight,
tick align=outside,
tick pos=left,
width=\figurewidth,
x grid style={white!69.0196078431373!black},
xlabel={Iterations},
xmin=-60, xmax=1260,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Landing Probability},
ymin=-0.022, ymax=0.462,
ytick style={color=black}
]
\addplot [semithick, color0]
table {%
0 0.02
1 0.02
2 0.02
3 0
4 0
5 0
6 0
7 0
8 0
9 0
10 0
11 0
12 0
13 0
14 0
15 0
16 0
17 0
18 0
19 0
20 0
21 0
22 0
23 0
24 0
25 0
26 0
27 0
28 0
29 0
30 0
31 0
32 0
33 0
34 0
35 0
36 0
37 0
38 0
39 0
40 0
41 0
42 0
43 0
44 0
45 0
46 0
47 0
48 0
49 0
50 0
51 0
52 0
53 0
54 0
55 0
56 0
57 0
58 0
59 0
60 0
61 0
62 0
63 0
64 0
65 0
66 0
67 0
68 0
69 0
70 0
71 0
72 0
73 0
74 0
75 0
76 0
77 0
78 0
79 0
80 0
81 0
82 0
83 0
84 0
85 0
86 0
87 0
88 0
89 0
90 0
91 0
92 0
93 0
94 0
95 0
96 0
97 0
98 0
99 0
100 0
101 0
102 0
103 0
104 0
105 0
106 0
107 0
108 0
109 0
110 0
111 0
112 0
113 0
114 0
115 0
116 0
117 0
118 0
119 0
120 0
121 0
122 0
123 0
124 0
125 0
126 0
127 0
128 0
129 0
130 0
131 0
132 0
133 0
134 0
135 0
136 0
137 0
138 0
139 0
140 0
141 0
142 0
143 0
144 0
145 0
146 0
147 0
148 0
149 0
150 0
151 0
152 0
153 0
154 0
155 0
156 0
157 0
158 0
159 0
160 0
161 0
162 0
163 0
164 0
165 0
166 0
167 0
168 0
169 0
170 0
171 0
172 0
173 0
174 0
175 0
176 0
177 0
178 0
179 0
180 0
181 0
182 0
183 0
184 0
185 0
186 0
187 0
188 0
189 0
190 0
191 0
192 0
193 0
194 0
195 0
196 0
197 0
198 0
199 0
200 0
201 0
202 0
203 0
204 0
205 0
206 0
207 0
208 0
209 0
210 0
211 0
212 0
213 0
214 0
215 0
216 0
217 0
218 0
219 0
220 0
221 0
222 0
223 0
224 0
225 0
226 0
227 0
228 0
229 0
230 0
231 0
232 0
233 0
234 0
235 0
236 0
237 0
238 0
239 0
240 0
241 0
242 0
243 0
244 0
245 0
246 0
247 0
248 0
249 0
250 0
251 0
252 0
253 0
254 0
255 0
256 0
257 0
258 0
259 0
260 0
261 0
262 0
263 0
264 0
265 0
266 0
267 0
268 0
269 0
270 0
271 0
272 0
273 0
274 0
275 0
276 0
277 0
278 0
279 0
280 0
281 0
282 0
283 0
284 0
285 0
286 0
287 0
288 0
289 0
290 0
291 0
292 0
293 0
294 0
295 0
296 0
297 0
298 0
299 0
300 0
301 0
302 0
303 0
304 0
305 0
306 0
307 0
308 0
309 0
310 0
311 0
312 0
313 0
314 0
315 0
316 0
317 0
318 0
319 0
320 0
321 0
322 0
323 0
324 0
325 0
326 0
327 0
328 0
329 0
330 0
331 0
332 0
333 0
334 0
335 0
336 0
337 0
338 0
339 0
340 0
341 0
342 0
343 0
344 0
345 0
346 0
347 0
348 0
349 0
350 0
351 0
352 0
353 0
354 0
355 0
356 0
357 0
358 0
359 0
360 0
361 0
362 0
363 0
364 0
365 0
366 0
367 0
368 0
369 0
370 0
371 0
372 0
373 0
374 0
375 0
376 0
377 0
378 0
379 0
380 0
381 0
382 0
383 0
384 0
385 0
386 0
387 0
388 0
389 0
390 0
391 0
392 0
393 0
394 0
395 0
396 0
397 0
398 0
399 0
400 0
401 0
402 0
403 0
404 0
405 0
406 0
407 0
408 0
409 0
410 0
411 0
412 0
413 0
414 0
415 0
416 0
417 0
418 0
419 0
420 0
421 0
422 0
423 0
424 0
425 0
426 0
427 0
428 0.06
429 0.06
430 0.06
431 0.06
432 0.06
433 0.06
434 0.06
435 0.06
436 0.06
437 0.06
438 0.06
439 0.06
440 0.06
441 0.06
442 0.06
443 0.06
444 0.06
445 0.06
446 0.06
447 0.06
448 0.06
449 0.06
450 0.06
451 0.06
452 0.06
453 0.06
454 0.06
455 0.06
456 0.06
457 0.06
458 0.06
459 0.06
460 0.06
461 0.06
462 0.06
463 0.06
464 0.06
465 0.06
466 0.06
467 0.06
468 0.06
469 0.06
470 0.06
471 0.06
472 0.06
473 0.06
474 0.06
475 0.06
476 0.06
477 0.06
478 0.06
479 0.06
480 0.06
481 0.06
482 0.06
483 0.06
484 0.06
485 0.06
486 0.06
487 0.06
488 0.06
489 0.06
490 0.06
491 0.06
492 0.06
493 0.06
494 0.06
495 0.06
496 0.06
497 0.06
498 0.06
499 0.06
500 0.06
501 0.06
502 0.06
503 0.06
504 0.06
505 0.06
506 0.06
507 0.06
508 0.06
509 0.06
510 0.06
511 0.06
512 0.06
513 0.06
514 0.06
515 0.06
516 0.06
517 0.06
518 0.06
519 0.06
520 0.06
521 0.06
522 0.06
523 0.06
524 0.06
525 0.06
526 0.06
527 0.06
528 0.06
529 0.06
530 0.06
531 0.06
532 0.06
533 0.06
534 0.06
535 0.06
536 0.06
537 0.06
538 0.06
539 0.06
540 0.06
541 0.06
542 0.06
543 0.06
544 0.06
545 0.06
546 0.06
547 0.06
548 0.06
549 0.06
550 0.06
551 0.06
552 0.06
553 0.06
554 0.06
555 0.06
556 0.06
557 0.06
558 0.06
559 0.06
560 0.06
561 0.06
562 0.06
563 0.06
564 0.06
565 0.06
566 0.06
567 0.06
568 0.06
569 0.06
570 0.06
571 0.06
572 0.06
573 0.06
574 0.06
575 0.06
576 0.06
577 0.06
578 0.06
579 0.06
580 0.06
581 0.06
582 0.06
583 0.06
584 0.06
585 0.06
586 0.06
587 0.06
588 0.06
589 0.06
590 0.06
591 0.06
592 0.06
593 0.06
594 0.06
595 0.06
596 0.06
597 0.06
598 0.06
599 0.06
600 0.06
601 0.06
602 0.06
603 0.06
604 0.06
605 0.06
606 0.06
607 0.06
608 0.06
609 0.06
610 0.06
611 0.06
612 0.06
613 0.06
614 0.06
615 0.06
616 0.06
617 0.06
618 0.06
619 0.06
620 0.06
621 0.06
622 0.06
623 0.06
624 0.06
625 0.06
626 0.06
627 0.06
628 0.06
629 0.06
630 0.06
631 0.06
632 0.06
633 0.06
634 0.06
635 0.06
636 0.06
637 0.06
638 0.06
639 0.06
640 0.06
641 0.06
642 0.06
643 0.06
644 0.06
645 0.06
646 0.06
647 0.06
648 0.06
649 0.06
650 0.06
651 0.06
652 0.06
653 0.06
654 0.06
655 0.06
656 0.06
657 0.06
658 0.06
659 0.06
660 0.06
661 0.06
662 0.06
663 0.06
664 0.06
665 0.06
666 0.06
667 0.06
668 0.06
669 0.06
670 0.06
671 0.06
672 0.06
673 0.06
674 0.06
675 0.06
676 0.06
677 0.06
678 0.06
679 0.06
680 0.06
681 0.06
682 0.06
683 0.06
684 0.06
685 0.06
686 0.06
687 0.06
688 0.06
689 0.06
690 0.06
691 0.06
692 0.06
693 0.06
694 0.06
695 0.06
696 0.06
697 0.06
698 0.06
699 0.06
700 0.06
701 0.06
702 0.06
703 0.06
704 0.06
705 0.06
706 0.06
707 0.06
708 0.06
709 0.06
710 0.06
711 0.06
712 0.06
713 0.06
714 0.06
715 0.06
716 0.06
717 0.06
718 0.06
719 0.06
720 0.06
721 0.06
722 0.06
723 0.06
724 0.06
725 0.06
726 0.06
727 0.06
728 0.06
729 0.06
730 0.06
731 0.06
732 0.06
733 0.06
734 0.06
735 0.06
736 0.06
737 0.06
738 0.06
739 0.06
740 0.06
741 0.06
742 0.06
743 0.06
744 0.06
745 0.06
746 0.06
747 0.06
748 0.06
749 0.06
750 0.06
751 0.06
752 0.06
753 0.06
754 0.06
755 0.06
756 0.06
757 0.06
758 0.06
759 0.06
760 0.06
761 0.06
762 0.06
763 0.06
764 0.06
765 0.06
766 0.06
767 0.06
768 0.32
769 0.32
770 0.32
771 0.32
772 0.32
773 0.32
774 0.32
775 0.32
776 0.32
777 0.32
778 0.32
779 0.32
780 0.32
781 0.32
782 0.32
783 0.32
784 0.32
785 0.32
786 0.32
787 0.32
788 0.32
789 0.32
790 0.32
791 0.32
792 0.32
793 0.32
794 0.32
795 0.32
796 0.32
797 0.32
798 0.32
799 0.32
800 0.32
801 0.32
802 0.32
803 0.32
804 0.32
805 0.32
806 0.32
807 0.32
808 0.32
809 0.32
810 0.32
811 0.32
812 0.32
813 0.32
814 0.32
815 0.32
816 0.32
817 0.32
818 0.32
819 0.32
820 0.32
821 0.32
822 0.32
823 0.32
824 0.32
825 0.32
826 0.32
827 0.32
828 0.32
829 0.32
830 0.32
831 0.32
832 0.32
833 0.32
834 0.32
835 0.32
836 0.32
837 0.32
838 0.32
839 0.32
840 0.32
841 0.32
842 0.32
843 0.32
844 0.32
845 0.32
846 0.32
847 0.32
848 0.32
849 0.32
850 0.32
851 0.32
852 0.32
853 0.32
854 0.32
855 0.32
856 0.32
857 0.32
858 0.32
859 0.32
860 0.32
861 0.32
862 0.32
863 0.32
864 0.32
865 0.32
866 0.32
867 0.32
868 0.32
869 0.32
870 0.32
871 0.32
872 0.32
873 0.32
874 0.32
875 0.32
876 0.32
877 0.32
878 0.32
879 0.32
880 0.32
881 0.32
882 0.32
883 0.32
884 0.32
885 0.32
886 0.32
887 0.32
888 0.32
889 0.32
890 0.32
891 0.32
892 0.32
893 0.32
894 0.32
895 0.32
896 0.32
897 0.32
898 0.32
899 0.32
900 0.32
901 0.32
902 0.32
903 0.32
904 0.32
905 0.32
906 0.32
907 0.32
908 0.32
909 0.32
910 0.32
911 0.32
912 0.32
913 0.32
914 0.32
915 0.32
916 0.32
917 0.32
918 0.12
919 0.12
920 0.12
921 0.12
922 0.12
923 0.12
924 0.12
925 0.12
926 0.12
927 0.12
928 0.12
929 0.12
930 0.12
931 0.12
932 0.12
933 0.12
934 0.12
935 0.12
936 0.12
937 0.12
938 0.12
939 0.12
940 0.12
941 0.12
942 0.12
943 0.12
944 0.12
945 0.12
946 0.12
947 0.12
948 0.12
949 0.12
950 0.12
951 0.12
952 0.12
953 0.12
954 0.12
955 0.12
956 0.12
957 0.12
958 0.12
959 0.12
960 0.12
961 0.12
962 0.12
963 0.12
964 0.12
965 0.12
966 0.12
967 0.12
968 0.12
969 0.12
970 0.12
971 0.12
972 0.12
973 0.12
974 0.12
975 0.12
976 0.12
977 0.12
978 0.12
979 0.12
980 0.12
981 0.12
982 0.12
983 0.12
984 0.12
985 0.12
986 0.12
987 0.12
988 0.12
989 0.12
990 0.12
991 0.12
992 0.12
993 0.12
994 0.12
995 0.12
996 0.12
997 0.12
998 0.12
999 0.12
1000 0.12
1001 0.12
1002 0.12
1003 0.12
1004 0.12
1005 0.12
1006 0.12
1007 0.12
1008 0.12
1009 0.12
1010 0.12
1011 0.12
1012 0.12
1013 0.12
1014 0.12
1015 0.12
1016 0.12
1017 0.12
1018 0.12
1019 0.12
1020 0.12
1021 0.12
1022 0.12
1023 0.12
1024 0.12
1025 0.12
1026 0.12
1027 0.12
1028 0.12
1029 0.12
1030 0.12
1031 0.12
1032 0.12
1033 0.12
1034 0.12
1035 0.12
1036 0.12
1037 0.12
1038 0.12
1039 0.12
1040 0.12
1041 0.12
1042 0.12
1043 0.12
1044 0.12
1045 0.12
1046 0.12
1047 0.12
1048 0.12
1049 0.12
1050 0.12
1051 0.12
1052 0.12
1053 0.12
1054 0.12
1055 0.12
1056 0.12
1057 0.12
1058 0.12
1059 0.12
1060 0.12
1061 0.12
1062 0.12
1063 0.12
1064 0.12
1065 0.12
1066 0.12
1067 0.12
1068 0.12
1069 0.12
1070 0.12
1071 0.12
1072 0.12
1073 0.12
1074 0.12
1075 0.12
1076 0.12
1077 0.12
1078 0.12
1079 0.12
1080 0.12
1081 0.12
1082 0.12
1083 0.44
1084 0.44
1085 0.44
1086 0.44
1087 0.44
1088 0.44
1089 0.44
1090 0.44
1091 0.44
1092 0.44
1093 0.44
1094 0.44
1095 0.44
1096 0.44
1097 0.44
1098 0.44
1099 0.44
1100 0.44
1101 0.44
1102 0.44
1103 0.44
1104 0.44
1105 0.44
1106 0.44
1107 0.44
1108 0.44
1109 0.44
1110 0.44
1111 0.44
1112 0.44
1113 0.44
1114 0.44
1115 0.44
1116 0.44
1117 0.44
1118 0.44
1119 0.44
1120 0.44
1121 0.44
1122 0.44
1123 0.44
1124 0.44
1125 0.44
1126 0.44
1127 0.44
1128 0.44
1129 0.44
1130 0.44
1131 0.44
1132 0.44
1133 0.44
1134 0.44
1135 0.44
1136 0.44
1137 0.44
1138 0.44
1139 0.44
1140 0.44
1141 0.44
1142 0.44
1143 0.44
1144 0.44
1145 0.44
1146 0.44
1147 0.44
1148 0.44
1149 0.44
1150 0.44
1151 0.44
1152 0.44
1153 0.44
1154 0.44
1155 0.44
1156 0.44
1157 0.44
1158 0.44
1159 0.44
1160 0.44
1161 0.44
1162 0.44
1163 0.44
1164 0.44
1165 0.44
1166 0.44
1167 0.44
1168 0.44
1169 0.44
1170 0.44
1171 0.44
1172 0.44
1173 0.44
1174 0.44
1175 0.44
1176 0.44
1177 0.44
1178 0.44
1179 0.44
1180 0.44
1181 0.44
1182 0.44
1183 0.44
1184 0.44
1185 0.44
1186 0.44
1187 0.44
1188 0.44
1189 0.44
1190 0.44
1191 0.44
1192 0.44
1193 0.44
1194 0.44
1195 0.44
1196 0.44
1197 0.44
1198 0.44
1199 0.44
1200 0.44
};
\end{axis}

\end{tikzpicture}

